Synthetic HI observations of spiral structure in the outer disk in galaxies

By means of 3D hydrodynamical simulations, in a separate paper we have discussed the properties of non-axisymmetric density wave trains in the outermost regions of galaxy disks, based on the picture that self-excited global spiral modes in the bright optical stellar disk are accompanied by low-amplitude short trailing wave signals outside corotation; in the gas, such wave trains can penetrate through the outer Lindblad resonance and propagate outwards, forming prominent spiral patterns. In this paper we present the synthetic 21~cm velocity maps expected from simulated models of the outer gaseous disk, focusing on the case when the disk is dominated by a two-armed spiral pattern, but considering also other more complex situations. We discuss some aspects of the spiral pattern in the gaseous periphery of galaxy disks noted in our simulations that might be interesting to compare with specific observed cases.

==> report.tex <==
We are thankful you for the stimulative and fruitful report by both reviewers. Majority of changes in the text are marked by bold.

We added a new table and figure 4.
Figures 4 and 5 from the previous version have been merged.


Reviewer: 2

Q. Section 4, on the methodology for computing the HI brightness temperature, has been much reduced, which is a good thing. It is however now a bit sketchy. I would recommend reintroducing, just for reference the formula for the optical depth (eq 4.10 in the original paper), and more importantly giving the numerical values used for the thermal and "turbulent" velocity dispersions, or how they are computed if they are non homogeneous across the disk.

A>>

Eq. 4.10 has been returned.

Computation of both velocity dispersion components is quite straightforwards. Thermal component of the gas velocity dispersion is calculated directly from the distribution of the gas temperature (in Kelvins), known from the dynamical simulations. Integrating the product of the velocity and the square of the density over all gas velocities along line of sight gives a velocity dispersion (or a second moment). 


Q. In the first paragraph of section 5, the description of the panels of fig. 4 does not seems to be consistent with the caption of the figure.

A>> Only last sentence in the first paragraph related to Fig 4. First part of paragraph is a discussion of the HI data cube which are shown in Fig 3.

Q. The effect of beam smearing is taken into account by smoothing on 700 pc. This choice of value should be supported by quoting an example of instrumental resolution (GMRT or other) and a typical distance to the galaxy.

A>>

For instance, in paper by Boomsma et al (2008), beam size is 22'' for velocity field (see Fig 2) where conversion unit is 60'' = 1.75 kpc (see Table 1 in Boomsma et al (2008)). Thus we can expect that for NGC 6946, 700 pc = 24'' which is comparable to our smoothing.  

Q. Nowhere quantitative values for the brightness temperatures are given. And yet the need for "deep integration" is mentioned in the discussion. A "back-of-the-envelope"  evaluation of the required integration time for at least one instrument, needed to exact some for in the interesting features would be most welcome. In particular the choice of the channel width is probably a important parameter.

A>> Of course channel width plays an important role in measuring of the velocity distribution. But it mostly important for extraction of the velocity and line profiles. However, for our basic conclusions it not a crucial factor.


Reviewer: 1


Q1. Column densities
Current HI observations with interferometers reach column densities of at most 1x10^19 cm^-2, these are in particular the lowest column densities reached in the papers quoted by the authors and also for the lowest resolution total HI maps, see e.g. Fig. 17 in Boomsma+ (2008).
In the models presented here the contours start from 1x10^18 cm^-2, it would much be better to start from 10^19 for a realistic comparison. 
Also please specify how the contours are incremented.

A>> Figures 4,5 were merged (now Figure 5). Column density contours now are in the range (1-15)x10^19 cm^-2 with corresponded several level ticks.

Q2. Position-velocity diagrams
The p-vs in Fig. 7 are puzzling. 
First, the unperturbed p-v shows emission at very low rotation velocities (down to -100 and +100 depending on the side). The authors state that this is due to thickness and asymmetric drift, but how thick is this disk? And if the disk is thick and flaring why is this emission especially visible in the inner rather than the outer parts?
To be honest, this looks like the p-v diagram of an edge-on galaxy, are you sure that you have extracted it along the major axis of your inclined galaxy? Or did you use a very thick slice? If it has to be compared to observations it should be extract from a slice along the major axis and very narrow (<= resolution) in the perpendicular direction, see e.g. Fig. 5 in Boomsma+ (2008). Also please try to plot realistic contours, it may be that the levels shown here are beyond detection with any instrument.

Second, the emission in the right panel departs to much from the rotation curve and it would make a huge difference for the global kinematics.
If I were to derive the rotation at 18 kpc from the centre using this datacube, I would get a value of about 60 km/s instead of 210 km/s! This cannot be true as rotation curves would not be flat anymore. In fact the curve from Fig. 7 right looks solid-body like out to about 40 kpc from the centre!
Again, the edge-on view would provide an explanation to this.

A>> Problem has been solved by more accurate alignment to the major axis and decreasing of the slice width. 

Q3. Models
The authors use more than one simulation and I think it could be useful to have a table summarizing their main features.
As far as I understand, the 4 models in Fig. 2 are: 1) m=1, 2) m=2 + high vel disp, 3) m=2 (normal vel dips?), 4) m=1,2,3
In Fig. 3 it's model 4, in Fig. 4 it's model 4 (top) and model 2? (bottom)?
Same in Fig. 6?

A>> All figures are now linked with corresponded parameters of galaxies.

Q. It is not clear to me how the higher velocity dispersion of model 2 was added? Is it higher temperature, or added random kinetic energy?

A>> It is only higher thermal component of the gas velocity dispersion (see Table 1).

Q. If I understand correctly in the model with "normal" velocity dispersion, there is no intrinsic turbulence added right? 

A>> For simplicity our models doesn't include initial intrinsic turbulence. 

Q. The authors say that sigma_v is a "superposition of thermal component and the random motion of the gas".
These random motions come from the instability and the shear I guess and it would be interesting to know how broad is a line profile in these simulations. Does it compare with the line profiles of the outer disks of sigma=6-7 km/s (FWHM=14-16 ams)?

A>> We added a new figure 4 with a line profiles for several positions in the galaxy. There is a sensible difference between line width in spirals and in the inter-arm region. Larger random motions in the vicinity of spirals arises due to shear flow and wiggle instability. In spirals we found FWHM values that you mentioned, but in the inter-arm regions random component of the velocity dispersion seems to be much smaller.

Q4. Figures
I suspect that the projection in Figs. 3 to 6 is for a disc inclined 60 degrees and not 30 along the l.o.s.

A>>

Q. What is the systemic velocity in Fig. 3? The channel at -150 km/s seems symmetrical to the channel at +210, strange. Also there is no emission at -220 km/s, why? 

A>> Systematic velocity is 0. Possible axisymmetry in the flux distribution can be the demonstration of non-axisymmetry of pattern in case of several modes imposed in simulations. 


Q. The same channel map shows emission after the arms have evolved, is this an effect of the evolution? Difficult to guess from the p-vs in Fig. 7.

A>> Yes. This is effect of evolution. Please see a new version of figure 7.

Q. Please specify the levels of the contours in Fig. 3, in some units.

A>> Done.

Q. Fig. 4 has been smoothed, right? please specify.

A>> Yes. Done.

Q. Fig. 4 and Fig. 5 bottom panels are identical, I do not think that it is necessary to repeat them.

A>> Ok. Fig 4 and 5 are merged.

Q. In Fig. 6, the top (left and middle) panels are slightly smaller than all the others.

A>> Corrected.
